Learning Augmented Energy Minimization via Speed Scaling

As power management has become a primary concern in modern data centers, computing resources are being scaled dynamically to minimize energy consumption. We initiate the study of a variant of the classic online speed scaling problem, in which machine learning predictions about the future can be integrated naturally. Inspired by recent work on learning-augmented online algorithms, we propose an algorithm which incorporates predictions in a black-box manner and outperforms any online algorithm if the accuracy is high, yet maintains provable guarantees if the prediction is very inaccurate. We provide both theoretical and experimental evidence to support our claims.

==> Conv_Alg_Experiments.tex <==

\begin{table}
\centering
\caption{The values under the Accurate and Random column are average competitive ratios over $5$ experiments while the last column gives the worse competitive ratio of each algorithm across 5 experiments. We used $m=20$, $M=80$, $s=5$ and $T = 20$.}
\vskip +0.15in
\label{table:normal regime results with convolution algorithm}
{\small
\begin{tabular}{lcccr}
\toprule
Algorithm & Accurate & Random & Misleading \\
\midrule
AVR     & 1.283 & 1.283 & 1.375 \\
BKP     & 8.118     & 8.118     & 8.897   \\
OA     & 1.216     & 1.216     & 1.334   \\
\hline
LAS, $\epsilon = 0.2$    & 1.088& 1.223& 1.632\\
CONV, $\epsilon = 0.2$    & 1.329& 1.375& 6.060\\
\hline
%%%%%
LAS, $\epsilon = 0.15$    & 1.061& 1.218& 1.687\\
CONV, $\epsilon = 0.15$    & 1.298& 1.599& 6.672\\
\hline
%%%%%
LAS, $\epsilon = 0.1$    & 1.038& 1.214& 1.722\\
CONV, $\epsilon = 0.1$    & 1.235& 1.912& 7.273\\
\hline
%%%%%
LAS, $\epsilon = 0.05$    & 1.009& 1.227& 1.766\\
CONV, $\epsilon = 0.05$    & 1.130& 2.282& 7.793\\
\hline
%%%%%
LAS, $\epsilon = 0.01$    & 1.009& 1.227& 1.766\\
CONV, $\epsilon = 0.01$    & 1.033& 2.867& 8.810\\
%%%%%
\bottomrule
\end{tabular}
}
\vskip -0.23in
\end{table}



==> Theoretical_analysis_reworked_again.tex <==
\section{Theoretical analysis (reworked again)}
\label{sec:Theoretical analysis}
In our analysis we give three different upper bounds on the value of the solution produced by our algorithm
(robustness, consistency, and smoothness). The smoothness bound implies that for consistency, but we
state it separately, as it is a particularly interesting case.
\begin{thm}\label{thm:analysis-main}
  With robustness parameter $O(\epsilon / \alpha)$
  the LAS algorithm satisfies the following guarantees.
  \begin{enumerate}
      \item Robustness (always):
        $O(\alpha/\epsilon)^{2\alpha} \OPT$
      \item Consistency (if the prediction is perfect): $(1 + \epsilon) \OPT$
      \item Smoothness (always):
      \begin{equation*}
        (1 + \epsilon) \OPT + O\left(\frac{\alpha}{\epsilon}\right)^{2\alpha} ||w - \tilde w ||_\alpha^\alpha
      \end{equation*}
  \end{enumerate}
\end{thm}
We prove in \iffullversion{Appendix~\ref{sec:lower_bounds}}{the full version of this paper} that an algorithm that is $(1+\epsilon)$-consistent cannot have a robustness better that $\Omega(\alpha/\epsilon)^{\alpha-1}$.

As before we assume w.l.o.g.\ that at each time $i$ exactly one job $J_i = (r_i, w_i)$ arrives.
This means $r_i = i$.
The algorithm runs a preprocessing step on the input which potentially rounds the jobs release times and $T$.
As in the description of the algorithm, we will denote by $J'_i = (r'_i, w'_i)$ the rounded job with $r'_i = i$.
One rounded job $J'_i$ may correspond to multiple jobs $J_{j}$ merged into one.
Note that by definition of the algorithm $w'_i$ can only be non-zero,
if $i$ is a multiple of $\max\{\epsilon T, 1\}$:
A multiple of $\epsilon T$ if $T > 1/\epsilon$ and therefore rounding is performed;
a multiple of $1$ if $T\le 1/\epsilon$ and no rounding is performed.
We write $T'$ for the rounded value of $T$ and $\OPT'$ for the optimal solution of the rounded instance.

A crucial observation for our analysis is that the optimum increases only marginally by the rounding.
More precisely, $\OPT' \le (1-3\epsilon)^{-\alpha} \OPT$.
The proof is by standard arguments and can be found
\iffullversion{in Appendix~\ref{sec:preprocessing}}{in the full version}.

\paragraph{Robustness.}
Recall, the algorithm schedules (part of) each job $j$ at speed at most $w'_j / (\epsilon^2 T')$
during some interval and then assigns the rest of it uniformly at speed
no greater than $w'_j / T'$.
In particular, the speed it runs $j$ is always bounded by $w'_j (1 + 1/\epsilon^2) / T'$.
This implies the speed never exceeds
$1 + 1/\epsilon^2$ times the speed of AVR. As we have proved that
AVR is $2^\alpha$-competitive (Theorem~\ref{thm:AVR_ratio}), the competitive ratio of
LAS is at most
$2^\alpha ((1/\epsilon)^2 + 1)^{\alpha} = O(1/\epsilon)^{2\alpha}$.
\paragraph{Consistency.}
We will show that if the prediction is correct,
the algorithm runs at speed at most $(1+\epsilon)$ times the speed in the optimal schedule
for the rounded instance,
that is to say, $s_{\mathrm{LAS}}(t) \le (1+\epsilon) s_{\OPT'}(t)$ for all $t$.

Assume in the following that the prediction is the true instance.
In particular, the rounded prediction is also the rounded true instance.
Consider some point of time $t$ and denote by $\hat s(t)$ the speed of the tentative schedule
derived from the rounded predicted instance in the beginning.
Schedule $\hat s$ is constructed by capping the speed of the optimal
solution for the predicted instance. Hence, we have $\hat s(t) \le s_{\OPT'}(t)$.
The speed $s_{\mathrm{LAS}}(t)$ is composed of (i) the speed of the tentative schedule
$\hat s(t)\le s_{\OPT'}(t)$ and (ii) some speed less than $w'_j / T'$
for each job $J'_j$
which is processed at a speed higher than $w'_j / (\epsilon^2 T')$ in $s_{\OPT'}$
and which has $r'_j \le t \le r'_j + T'$.
The total number of the jobs from (ii) is bounded by $1/\epsilon$, since
rounded jobs arrive only at multiples of $\max\{\epsilon T, 1\}$ and $T' \le T$.
We argue that for each of these jobs $w'_j / T' \le \epsilon^2 s_{\OPT'}(t)$.

Consider one such job $j$. Recall, there is some time $t'$ where $J'_j$ is run at a speed
$s' > w'_j / (\epsilon^2 T')$ in $s_{\OPT'}$.
At the same time we know by Proposition~\ref{optimality_conditions}
that $s'\le s_{\OPT'}(t)$.
It follows that $w'_{j} / T' < \epsilon^2 s_{\OPT'}(t)$.

The speed of $\epsilon^2 s_{\OPT'}(t)$ for each of the at most $1/\epsilon$ many jobs that intersect with $t$
together with $s_{\OPT'}(t)$ as by (i) yields
\begin{equation*}
    s_{\mathrm{LAS}}(t) \le \left(1 + \frac{\epsilon^2}{\epsilon}\right)s_{\OPT'}(t) \le (1 + \epsilon) s_{\OPT'} (t).
\end{equation*}
Integrating over $t$ implies that the cost of the LAS schedule is at most
$(1+\epsilon)^\alpha \OPT' \le (1 + O(\epsilon))^\alpha \OPT$.

\paragraph{Smoothness.} 
For the dependency on the prediction error, we use the following inequality.
 For all $a,b\geq 0$ and $0 < \delta \le 1$ it holds that
 \begin{equation}
 (a+b)^\alpha\leq (1+\delta)^\alpha a^\alpha + \left(\frac{2}{\delta}\right)^\alpha b^\alpha . \label{eq:combine}
 \end{equation}
 This follows from a trivial case distinction
 on $b \le \delta a$.
 We will first relate the cost of the LAS schedule to the optimum of the predicted
 instance. Then we will relate the latter to the actual optimum.
 In the following, we will denote by $s_{\mathrm{LAS}}(t, w, \tilde w)$ the speed of the \textsc{LAS} schedule
 on instance $w$ with prediction $\tilde w$. Similarly, we define $s_{\mathrm{AVR}}(t, w)$ and $s_{\mathrm{OPT}}(t, w)$ for the AVR schedule and the optimal schedule. Note that here the prediction is omitted,
 since these algorithms do not depend on it.
 
 Define $w^+_i=\max\left(0,w_i-\tilde w_i \right)$ as the additional work arriving at time $i$ compared to the prediction (or $0$, if it is less). Likewise, let $w^-_i$ be the decrease in work or $0$.
 Clearly, $w - w^+$ (componentwise)
 forms a valid instance with $0 \le w_i - w^+_i \le \tilde w_i$ for all $i$.
 For the upcoming proof we are going to rely on the fact
 that the schedule produced by LAS is exactly the same as if the
 algorithm was run with $w - w^+$ as the true instance and $w^+$ was independently rounded then 
 scheduled using AVR. In other words, for all $t$ it holds that
 \begin{equation*}
     s_{\mathrm{LAS}}(t, w, \tilde w) = s_{\mathrm{LAS}}(t, w - w^+, \tilde w) + s_{\mathrm{AVR}}(t, (w^+)') .
 \end{equation*}

 It is easy to see by the behavior of LAS that the speed can only decrease,
 if the actual instance is smaller. In particular,
 $s_{\mathrm{LAS}}(t, w - w^+, \tilde w) \le s_{\mathrm{LAS}}(t, \tilde w, \tilde w)$ for all $t$.
 By the analysis of consistency, we know that 
 $ s_{\mathrm{LAS}}(t, \tilde w, \tilde w) \le (1 + \epsilon) s_{\OPT}(t, (\tilde w)')$ for all $t$.
 
 We then claim that the following holds for any instance $w$ and time $t$.
 
 \begin{equation}\label{rounding_avr}
     s_{\mathrm{AVR}}(t,w')\leq \frac{1}{1-2\epsilon}\cdot s_{\mathrm{AVR}}(t,w)
 \end{equation}{}
 
 For the proof notice that each job in the rounded instance $w'$ consists in some jobs from $w$ aggregated together. Let us call $w'_i$ the rounded job and $\{w_1,\ldots ,w_j\}$ the jobs in $w$ that are aggregated into $w'_i$. Since the support of each job $w_1,\ldots ,w_j$ is shrunk by a multiplicative factor of $(1-2\epsilon)$ then the average rate speed for $w'_i$ is at most $\frac{1}{1-2\epsilon}$ times the sum of the average rate speeds for each job in $w_1,\ldots w_j$. Hence the claim.

 Furthermore, since $|\cdot|^\alpha$ is a convex function, we get
 \begin{multline*}
  \int s_{\mathrm{AVR}}(t, w^+)^\alpha dt = \int \left(\frac 1 T \sum_{j\in [t-T,t]}w_j^+ \right)^\alpha dt \\
  \le \int \frac 1 T \sum_{j\in [t-T,t]}(w_j^+)^\alpha dt
  =\sum_j \frac 1 T \int_j^{j+T} (w_j^+)^\alpha dt
 \end{multline*}
 and the right hand side is exactly $||w^+||_\alpha^\alpha$. Using (\ref{eq:combine}) and (\ref{rounding_avr}) we conclude
 \begin{align*}
     &\int s_{\textrm{LAS}}(t, w, \tilde w)^\alpha dt \\
     &\leq (1+\epsilon^2)^\alpha(1 + \epsilon^2 T)^\alpha\int s_{\OPT}(t, \tilde w)^\alpha dt \\
     &\quad + \left(\frac{2}{\epsilon^2} \right)^\alpha  \int s_{\mathrm{AVR}}^+(t, (w^+)')^\alpha dt \\
     &\le (1 + O(\epsilon^2 T))^\alpha \OPT(\tilde w) + O\left(\frac{1}{\epsilon} \right)^{2\alpha} ||w^+||_\alpha^\alpha .
 \end{align*}
 It remains to relate $\OPT(\tilde w)$ to $\OPT(w)$.
 This can be done by reversing the roles of the predicted and actual instance. Clearly, by running in parallel the schedules $s_{\OPT}(t, w)$ and $s_{\mathrm{AVR}}(t, w^-)$,
 we have a feasible schedule for $\Tilde w$. Hence, by the same arguments,
 \begin{multline*}
    \OPT(\Tilde{w}) \leq \int \left(s_{\OPT}(t, w)+s_{\mathrm{AVR}}(t, w^-) \right)^\alpha dt \\
    \leq (1+\epsilon^2)^\alpha \OPT(w) + O\left(\frac{1}{\epsilon}\right)^{2\alpha} ||w^-||_\alpha^\alpha .
 \end{multline*}
 Combining all inequalities we bound the cost of the LAS schedule by
 \begin{equation*}
     (1+O(\epsilon^2 T))^{\alpha}\OPT + O\left(\frac{1}{\epsilon}\right)^{2\alpha} ||w - \tilde w||_\alpha^\alpha .
 \end{equation*}

==> old_theoretical_analysis_section.tex <==

\section{Theoretical analysis}
\label{sec:Theoretical analysis}
In our analysis we give three different upper bounds on the value of the solution produced by our algorithm
(robustness, consistency, and smoothness). The smoothness bound implies that for consistency, but we
state it separately, as it is a particularly interesting case.
\begin{thm}\label{thm:analysis-main}
  With robustness parameter $O(\epsilon / \alpha)$
  the LAS algorithm satisfies the following guarantees.
  \begin{enumerate}
      \item Robustness (always):
        $O(\alpha/\epsilon)^{2\alpha} \OPT$
      \item Consistency (if the prediction is perfect): $(1 + \epsilon) \OPT$
      \item Smoothness (always):
      \begin{equation*}
        (1 + \epsilon) \OPT + O\left(\frac{\alpha}{\epsilon} \max\left\{T, \frac \alpha \epsilon\right\}\right)^{\alpha} ||w - \tilde w ||_\alpha^\alpha
      \end{equation*}
  \end{enumerate}
\end{thm}
We prove in \iffullversion{Appendix~\ref{sec:lower_bounds}}{the full version of this paper} that an algorithm that is $(1+\epsilon)$-consistent cannot have a robustness better that $\Omega(\alpha/\epsilon)^{\alpha-1}$.

Our analysis is split in two parts. First, we analyse the guarantees of the algorithm
without preprocessing (that consists in the rounding procedure):
\begin{lem}\label{lem:no-preprocessing}
Without preprocessing the algorithm produces a solution of cost at most $O(1/\epsilon)^{2\alpha} \OPT$.
Regarding the prediction, the cost is always bounded by $(1 + O(\epsilon^2 T))^\alpha \OPT + O(1/\epsilon)^{2\alpha} ||w - \tilde w||_\alpha^\alpha$.
\end{lem}
Afterwards, we consider the effect of the preprocessing
and combining them with Lemma~\ref{lem:no-preprocessing} we
arrive at the statements of Theorem~\ref{thm:analysis-main}.
\subsection{Analysis without preprocessing}
\paragraph{Robustness.}
Recall, the algorithm schedules (part of) each job $j$ at speed at most $w_j / (\epsilon^2 T)$
during some interval and then assigns the rest of it uniformly at speed
no greater than $w_j / T$.
In particular, the speed it runs $j$ is always bounded by $w_j (1 + 1/\epsilon^2) / T$.
This implies the speed never exceeds
$1 + 1/\epsilon^2$ times the speed of AVR. As we have proved that
AVR is $2^\alpha$-competitive (Theorem~\ref{thm:AVR_ratio}), the competitive ratio of
LAS is at most
$2^\alpha ((1/\epsilon)^2 + 1)^{\alpha} = O(1/\epsilon)^{2\alpha}$.
\paragraph{Consistency.}
We will show that if the prediction is correct,
the algorithm runs at speed at most $(1+\epsilon^2 T)$ times the speed in the optimal schedule,
that is, $s_{\mathrm{LAS}}(t) \le (1+\epsilon^2 T) s_{\OPT}(t)$ for all $t$.

Consider some point of time $t$ and denote by $\hat s(t)$ the speed of the tentative schedule
derived from the predicted instance in the beginning. Since the predicted instance
is also the true instance and $\hat s$ is constructed by capping the speed of the optimal
solution for the predicted instance, we know that $\hat s(t) \le s_{\OPT}(t)$.
The speed $s_{\mathrm{LAS}}(t)$ is composed of (i) the speed of the tentative schedule
$\hat s(t)\le s_{\OPT}(t)$ and (ii) some speed less than $w_j / T$
for each job $j$
which is processed at a speed higher than $w_j / (\epsilon^2 T)$ in the optimal schedule
and which has $r_j \le t \le r_j + T$.
The total number of the jobs from (ii) is bounded by $T$, since we assume that
at each integral time at most one job arrives.
We argue that for each of these jobs $w_j / T \le \epsilon^2 s_{\OPT}(t)$.

Consider one such job $J'_j$. Recall, there is some time $t'$ where $j$ is run at a speed
$s' > w_j / (\epsilon^2 T)$ in the optimal solution.
At the same time we know by Proposition~\ref{optimality_conditions}
that $s'\le s_{\OPT}(t)$.
It follows that $w_{j} / T < \epsilon^2 s_{\OPT}(t)$.

The speed of $\epsilon^2 s_{\OPT}(t)$ for each of the at most $T$ many jobs that intersect with $t$
together with $s_{\OPT}(t)$ as by (i) yields $s_{\mathrm{LAS}}(t) \le (1 + \epsilon^2 T)s_{\OPT}(t)$.
Integrating over $t$ implies that the competitive ratio is at most
$(1+\epsilon^2 T)^\alpha$.

\paragraph{Smoothness.} 
For the dependency on the prediction error, we use the following inequality.
 For all $a,b\geq 0$ and $0 < \delta \le 1$ it holds that
 \begin{equation}
 (a+b)^\alpha\leq (1+\delta)^\alpha a^\alpha + \left(\frac{2}{\delta}\right)^\alpha b^\alpha . \label{eq:combine}
 \end{equation}
 This follows from a trivial case distinction
 on $b \le \delta a$.
 We will first relate the cost of the LAS schedule to the optimum of the predicted
 instance. Then we will relate the latter to the actual optimum.
 In the following, we will denote by $s_{\mathrm{LAS}}(t, w, \tilde w)$ the speed of the \textsc{LAS} schedule
 on instance $w$ with prediction $\tilde w$. Similarly, we define $s_{\mathrm{AVR}}(t, w)$ and $s_{\mathrm{OPT}}(t, w)$ for the AVR schedule and the optimal schedule. Note that here the prediction is omitted,
 since these algorithms do not depend on it.
 
 Define $w^+_i=\max\left(0,w_i-\tilde w_i \right)$ as the additional work arriving at time $i$ compared to the prediction (or $0$, if it is less). Likewise, let $w^-_i$ be the decrease in work or $0$.
 Clearly, $w - w^+$ (componentwise)
 forms a valid instance with $0 \le w_i - w^+_i \le \tilde w_i$ for all $i$.
 For the upcoming proof we are going to rely on the fact
 that the schedule produced by LAS is exactly the same as if the
 algorithm was run with $w - w^+$ as the true instance and $w^+$ was independently
 scheduled using AVR. In other words, for all $t$ it holds that
 \begin{equation*}
     s_{\mathrm{LAS}}(t, w, \tilde w) = s_{\mathrm{LAS}}(t, w - w^+, \tilde w) + s_{\mathrm{AVR}}(t, w^+) .
 \end{equation*}

 It is easy to see by the behavior of LAS that the speed can only decrease,
 if the actual instance is smaller. In particular,
 $s_{\mathrm{LAS}}(t, w - w^+, \tilde w) \le s_{\mathrm{LAS}}(t, \tilde w, \tilde w)$ for all $t$.
 By the analysis of consistency, we know that 
 $ s_{\mathrm{LAS}}(t, \tilde w, \tilde w) \le (1 + \epsilon^2 T) s_{\OPT}(t, \tilde w)$ for all $t$.

 Furthermore, since $|\cdot|^\alpha$ is a convex function, we get
 \begin{multline*}
  \int s_{\mathrm{AVR}}(t, w^+)^\alpha dt = \int \left(\frac 1 T \sum_{j\in [t-T,t]}w_j^+ \right)^\alpha dt \\
  \le \int \frac 1 T \sum_{j\in [t-T,t]}(w_j^+)^\alpha dt
  =\sum_j \frac 1 T \int_j^{j+T} (w_j^+)^\alpha dt
 \end{multline*}
 and the right hand side is exactly $||w^+||_\alpha^\alpha$. Using (\ref{eq:combine}) we conclude
 \begin{align*}
     &\int s_{\textrm{LAS}}(t, w, \tilde w)^\alpha dt \\
     &\leq (1+\epsilon^2)^\alpha(1 + \epsilon^2 T)^\alpha\int s_{\OPT}(t, \tilde w)^\alpha dt \\
     &\quad + \left(\frac{2}{\epsilon^2} \right)^\alpha  \int s_{\mathrm{AVR}}^+(t, w^+)^\alpha dt \\
     &\le (1 + O(\epsilon^2 T))^\alpha \OPT(\tilde w) + O\left(\frac{1}{\epsilon} \right)^{2\alpha} ||w^+||_\alpha^\alpha .
 \end{align*}
 It remains to relate $\OPT(\tilde w)$ to $\OPT(w)$.
 This can be done by reversing the roles of the predicted and actual instance. Clearly, by running in parallel the schedules $s_{\OPT}(t, w)$ and $s_{\mathrm{AVR}}(t, w^-)$,
 we have a feasible schedule for $\Tilde w$. Hence, by the same arguments,
 \begin{multline*}
    \OPT(\Tilde{w}) \leq \int \left(s_{\OPT}(t, w)+s_{\mathrm{AVR}}(t, w^-) \right)^\alpha dt \\
    \leq (1+\epsilon^2)^\alpha \OPT(w) + O\left(\frac{1}{\epsilon}\right)^{2\alpha} ||w^-||_\alpha^\alpha .
 \end{multline*}
 Combining all inequalities we bound the cost of the LAS schedule by
 \begin{equation*}
     (1+O(\epsilon^2 T))^{\alpha}\OPT + O\left(\frac{1}{\epsilon}\right)^{2\alpha} ||w - \tilde w||_\alpha^\alpha .
 \end{equation*}

\paragraph{Effects of preprocessing.}
In the preprocessing the algorithm rounds release times and deadlines.
This may increase the cost of the optimal solution. However, we show that
this increase is only by a marginal factor of no more than
$(1-3\epsilon)^{-\alpha}$.
At the same time the number of jobs $J_j$ intersecting with a point of time $t$, that
is $r_j \le t \le r_j + T$, is decreased to at most $1/\epsilon$. Finally,
the error of the prediction,
$||w - \tilde w||_\alpha^\alpha$ increases by a factor less than $(\epsilon T)^{\alpha-1}$.
The proofs are by standard arguments, which can be found
\iffullversion{in Appendix~\ref{sec:preprocessing}}{in the full version}.

We notice that the bounds of the form $(1 + \epsilon^2 T)$ from Lemma~\ref{lem:no-preprocessing}
improve to $(1 + \epsilon)$, since only $1/\epsilon$ jobs intersect on a given time.
Considering the remaining effects of preprocessing, we calculate that
the guarantees of Lemma~\ref{lem:no-preprocessing} change to
$O(1/\epsilon)^{2\alpha} \OPT$ (robustness) and for consistency/smoothness
\begin{equation*}
(1+O(\epsilon))^\alpha \OPT + O\left(\frac{1}{\epsilon}\max\left\{T, \frac 1 \epsilon\right\}\right)^{\alpha} ||w - \tilde w||_\alpha^\alpha.
\end{equation*}
Scaling down $\epsilon$ by dividing it with a factor $O(\alpha)$ gives the
tradeoff as in Theorem~\ref{thm:analysis-main}.


